Theoretical analysis of git bisect

In this paper, we consider the problem of finding a regression in a version control system (VCS), such as git. The set of versions is modelled by a Directed Acyclic Graph (DAG) where vertices represent versions of the software, and arcs are the changes between different versions. We assume that somewhere in the DAG, a bug was introduced, which persists in all of its subsequent versions. It is possible to query a vertex to check whether the corresponding version carries the bug. Given a DAG and a bugged vertex, the Regression Search Problem consists in finding the first vertex containing the bug in a minimum number of queries in the worst-case scenario. This problem is known to be NP-complete. We study the algorithm used in git to address this problem, known as git bisect. We prove that in a general setting, git bisect can use an exponentially larger number of queries than an optimal algorithm. We also consider the restriction where all vertices have indegree at most 2 (i.e. where merges are made between at most two branches at a time in the VCS), and prove that in this case, git bisect is a $\frac{1}{\log_2(3/2)}$-approximation algorithm, and that this bound is tight. We also provide a better approximation algorithm for this case. Finally, we give an alternative proof of the NP-completeness of the Regression Search Problem, via a variation with bounded indegree.

==> figures/fibonacci_tree_F0.tex <==
\begin{tikzpicture}
    [
        scale=.6,
        auto=left,
        every node/.style={circle,draw,scale=0.8},
        minimum size=0.75cm,
        text opacity=0,
    ]

    \node[draw=none] (empty1) at (-2,9) {1};
    \node[draw=none] (empty2) at (-2,8) {1};
    \node[draw=none] (empty3) at (-2,7) {1};
    
\end{tikzpicture}

